T3P: Demystifying Low-Earth Orbit Satellite Broadband

The Internet is going through a massive infrastructural revolution with the advent of low-flying satellite networks, 5/6G, WiFi7, and hollow-core fiber deployments. While these networks could unleash enhanced connectivity and new capabilities, it is critical to understand the performance characteristics to efficiently drive applications over them. Low-Earth orbit (LEO) satellite mega-constellations like SpaceX Starlink aim to offer broad coverage and low latencies at the expense of high orbital dynamics leading to continuous latency changes and frequent satellite hand-offs. This paper aims to quantify Starlink's latency and its variations and components using a real testbed spanning multiple latitudes from the North to the South of Europe. We identify tail latencies as a problem. We develop predictors for latency and throughput and show their utility in improving application performance by up to 25%. We also explore how transport protocols can be optimized for LEO networks and show that this can improve throughput by up to 115% (with only a 5% increase in latency). Also, our measurement testbed with a footprint across multiple locations offers unique trigger-based scheduling capabilities that are necessary to quantify the impact of LEO dynamics.

==> design.tex <==
\vspace{-0.05in}
\section{Design, architecture, \& Implementation}
\label{sec:design}

%\subsection{Challenges} -- 
%THESE DO NOT SEEM TO BE DESIGN CHALLENGES. ALSO, WE DISCUSS COST UNDER DISCUSSION SECTION.
%Building a LEO satellite network testbed poses the following significant challenges: (i) StarLink is the largest LEO satellite network, but it is still not widely available. Moreover, the cost of a LEO node is relatively high: Starlink Internet costs \$110, \$135, and \$500 monthly subscription for regular use, RV use, and business use with \$500-\$2500 one-time equipment cost. This makes it challenging to construct a large-scale testbed. (ii) It is the first of kind of LEO satellite network. We do not have a prior example testbed to follow. (iii) Developing scavenger mode and trigger-based experiment scheduling are very useful but non-trivial.   



\begin{figure*}[t]
  \centering
  \subfigure[]{\label{fig:leopard_design}
    \includegraphics[width=0.75\textwidth]{figures/design/leopard_design.png}}
  \subfigure[]{\label{fig:leopard_terminal}
    \includegraphics[width=0.1\textwidth]{figures/design/redmond_node.png}}
  \vspace{-0.2in}
  \caption{(a) \projectname{}'s broad design and building blocks. (b) A user terminal deployed in the US ($47\degree${}N) with a clear view of the sky. \db{This and the corr. discussion should mostly move to the appendix.}}
  \vspace{-0.15in}
\end{figure*}

In this section, we touch upon the current design, architecture and implementation of \projectname{}. As with any other large-scale testbeds, we anticipate evolution with scale.

\subsection{Broad design}

Fig.~\ref{fig:leopard_design} explains \projectname{} in a nutshell. Let us touch upon the individual key components below.

\parab{Users} are the customers of the testbed. Users could submit network/application-level experiments to \projectname{}, request a schedule and a set of measurement clients and servers to run these experiments on, and view the results dashboard. %PlanetLab scaled up by requiring each user's university to contribute infrastructure. Unfortunately, this is not feasible for \projectname{} because LEO connectivity could be geographically restricted and may not be available in the home regions of the researchers.  Therefore,  users do not necessarily contribute resources to \projectname{}. Instead, 
User-submitted experiments need to be reviewed by an independent committee to verify the experiment intent and whether the current testbed can host the experiments.

\parab{Cloud orchestrator} is responsible for scheduling experiments across measurement clients and servers, managing schedule conflicts, and monitoring measurement node health. It maintains a database of nodes (and node health), and scheduled experiments and node mappings. When a new experiment scheduling request arrives at the orchestrator, it accepts/rejects the requested schedule after checking against existing schedules. Individual measurement clients could autonomously reschedule experiments in order to accommodate scavenger mode, as described above, and are responsible for notifying the cloud orchestrator of such updates. The orchestrator makes sure that the users could run experiments and gather results on \projectname{} without touching the individual nodes deployed.

\parab{Measurement servers} are deployed on public cloud. For client-server measurement experiments like \texttt{iperf}~\cite{iperf}, measurement clients could reach out to these servers. The server daemon receives an experiment schedule from the cloud orchestrator, downloads the necessary artifacts, and sets up the local environment (if needed) before the client requests arrive. The server-side experiment is responsible for pushing the results to the cloud for passive analysis. We rely on community resources to deploy these servers at scale.

\parab{Measurement clients} need to be deployed across the globe to run \projectname{} experiments. %and understand the impact of various factors like cell congestion, weather, geometry, GEO arc-avoidance, etc. 
A client node consists of an LEO user terminal %(involves a one-time hardware cost and regular subscription charges) 
with a reasonably clear view of the sky (see Fig.~\ref{fig:leopard_terminal}), and a host (could be standard workstations, Raspberry Pi~\cite{rasp_pi}, or more capable edge devices like Azure Stack Edge~\cite{ase} or Intel NUC~\cite{intel_nuc}) behind the terminal that could access the Internet via the user terminal. Some of these clients could also have alternate terrestrial Internet connectivity which, when available, could be used to compare against LEO connectivity. We envision universities, enterprises, and individual LEO customers dedicating a slice of their resources to \projectname{}. These clients register with the cloud orchestrator and send regular heartbeat signals to make sure that the orchestrator is aware of the node's health. When an experiment schedule request involves a client node, the orchestrator checks the node health and the database of already scheduled experiments on this node. If permissible, the orchestrator issues a new experiment request to this client which, upon receiving the request, downloads the necessary artifacts and sets up the local environment, as needed, to run the same.

\parab{Cloud storage} receives measurement data from both measurement clients and servers. The storage is hierarchically structured into directories such that it is straightforward to navigate to a specific instance of an experiment on a measurement node. The cloud orchestrator leverages a post-processing library that fetches data from this cloud storage and generates insights (plots, visuals, etc.) to be displayed on the user dashboard.

\parab{} \projectname{} is envisioned to be a community-driven testbed. Hence, the design relies on large enterprises or universities dedicating/sponsoring cloud resources for hosting the orchestrator, measurement servers, and cloud storage services.

\begin{figure}[tbh]
        \begin{center} \includegraphics[width=0.5\columnwidth]{figures/design/leopard-arch-diagram.jpg}
                \vspace{-0.18in}
                \caption{\projectname{}'s high-level architecture. \db{This and the corr. discussion should mostly move to the appendix.}
                }
                \label{fig:architecture}
        \end{center}
        %\vspace{-0.3in}
\end{figure}

\subsection{Architectural building blocks}

Fig.~\ref{fig:architecture} shows the high-level architecture of \projectname{}. The user interface is currently a Command Line Interface (CLI), with users being able to schedule new experiments and specify triggers, check measurement client and server status, and fetch experiment results. %\fix{``Will be done soon'' does not cut it for a submitted paper draft. let's remove this kind of language.} 
The cloud orchestrator manages $2$ core services at scale -- $1$. scheduling experiments on clients and servers, and $2$. managing measurement servers, nodes, and user access to resources. It leverages the cloud data store for persisting experiment schedules, user and node details, and consuming experiment data coming from individual clients and servers to the results store. The measurement clients and servers run the following services -- $1$. a scheduler service which consumes experiment schedules published by the cloud orchestrator and notifies the local cron daemon of such schedules; $2$. the experiment executor container that runs the network experiment according to user-specified and cloud orchestrator-approved schedules; $3$. the terminal data consumer service that continually consumes provider-specific disclosed data from the user terminal which could then be used for further analysis, trigger-based scheduling, etc.; and $4$. the heartbeat service which sends heartbeat data regularly to the cloud orchestrator.

\parab{Clients behind NATs and firewalls} The measurement clients are often behind NATs and firewalls. %thus making it hard for the cloud orchestrator to communicate commands and experiment requests. 
Hence, the cloud orchestrator piggybacks experiment schedules and other commands to clients and servers on the heartbeat response. %Even if \projectname{} scales to hundreds of nodes, this piggybacking is expected to not generate significant query overhead. If it scales even beyond, it could move to a publish-subscribe pattern for these control commands.}
%\fix{Separate question is how many nodes will we eventually need. Can we do some back of envelope calculation that if we have x nodes per latitude we can see most of the dynamics htat occur in all of the orbital shells that Starlink has?}

\parab{Lightweight isolation} \projectname{} runs experiments on containers~\cite{container}. Containers are lightweight (same OS kernel; isolated user-space processes) and offer faster start-ups than full-fledged virtual machines. Also, containers could be hosted on public repositories (like Docker Hub~\cite{docker_hub}) which makes deployment at scale easier. However, containers do not allow users to tinker around with low-level features (like deploying a kernel-based congestion control).

%\debopam{\projectname{} dockerizes all experiments. Docker containers offer virtualization of the operating system. These are lightweight compared to virtual machines but offer similar isolations. Dockerized experiments are hosted publicly on Docker Hub~\fix{\cite{docker_hub}}, which could be lazy-downloaded by measurement clients and servers on receiving relevant commands from the cloud orchestrator.} 
%\fix{[Shubham] We can convey something along the lines of following:
%The current implementation of LEOpard allows execution of containerized experiments. Containers are a lightweight solution to experiment isolation as they provide virtualization at the OS-layer as opposed to Virtual Machines that offer virtualization at the level of hardware. As such, containers enable a shorter experimentation cycle owing to smaller size, faster start-up times, and less resource-intensive. Moreover, containers can be hosted on container repositories like Dockerhub which makes the experiment deployment easier. Containerization suffices for most experiments (including all the experiments presented in this paper). However, it does not allow for the experimentors to play around with lower-level features (ex, developing kernel based CCs). The expansion of LEOpard to such use-cases is left for the future.}

\parab{Explicit overhead declaration} 
Experiments are marked as either overhead or no-overhead. No-overhead experiments include ping latency measurements, traceroute, etc., which can run in the background with minimal impact on other experiments and traffic. Overhead experiments can run in parallel with no-overhead experiments but not with other overhead experiments. The terminal data consumer service, on detecting user traffic, triggers scavenger mode only for overhead experiments.
%Experiments are explicitly marked as overhead or no-overhead at the time of adding them to the testbed's library of experiments on Docker Hub. Ping latency measurements, traceroute experiments, and those which consume the user terminal generated data are marked as no-overhead --these experiments can run in the background with minimal impact on other overhead experiments and user traffic. Overhead experiments could be scheduled in parallel to multiple non-overhead experiments but not to other overhead experiments. Also, when user traffic is detected by the terminal data consumer service, only overhead experiments need to be preempted/rescheduled to enter the scavenger mode.


==> implementation.tex <==
\vspace{-0.05in}
\subsection{Current Implementation}
\label{sec:implementation}

%\fix{[Shubham] Things to touch upon: Which cloud service? Details of the cloud orchestrator, the interfaces with users, measurement servers and clients, the frequency of communications. How is an experiment scheduled (step-by-step). The different cloud datastores. List of libraries used.}

The Azure-hosted cloud orchestrator exposes gRPC~\cite{grpc} APIs to the user interface and measurement clients/servers. A MongoDB~\cite{mongodb} server on Azure hosts the Experiment and User/Node DB (see Fig.~\ref{fig:architecture}). All experiment data are stored on Azure Blob Storage~\cite{azure_blob_storage} (results store). Users leverage orchestrator-exposed APIs to (a) submit experiments and schedules, (b) specify experiment parameters, measurement clients, and servers, (c) mark experiments as overhead (bandwidth-heavy) or no-overhead (like latency probes), and (d) monitor experiment status. The cloud orchestrator is in charge of verifying the experiment configuration, checking for scheduling conflicts, and verifying trigger strings (for trigger-based scheduling), if any. At each measurement node, the heartbeat service sends regular ($10$s) heartbeats to the cloud orchestrator and receives piggybacked experiment schedules, which are then handed over to the node-local scheduler service. Next, the scheduler updates the local crontab to invoke the experiment executor according to the schedule  and with the specified job parameters. The executor service is in charge of launching individual experiments, streaming logs, monitoring (and killing, if needed) the execution, and uploading the logs to the results store. Once uploaded, the executor deletes local logs and notifies the cloud orchestrator of the termination. The cloud orchestrator then terminates the measurement server stub, if any.

%The Cloud Orchestrator exposes a gRPC \fix{\cite{?}} service for communication with the measurement nodes and the user interface. Datastore (Experiment and User/Node DB) is a MongoDB server. The experiment data is stored in an Azure Blob Storage (Results Store). 

%The scheduler service in the node polls the orchestrator at a fixed time interval of 10 seconds to get experiments to be scheduled on the node. The scheduler then updates the local cron tab to invoke the experiment executor at the specified cron schedule and with the specified job parameters. The executor executes the job in 3 stages -- 1. \textbf{Deployment stage}: the executor prepares the environment for experiment execution. This involves downloading/updating the experiment containers from remote repository and setting up the measurement server (if any), 2. \textbf{Execution Stage}: the executor launches the experiment container and streams the stdout/stderr logs. The executor also monitors the execution time of the containers and kills the container if the execution time exceeds the allocated time. 3. \textbf{Finishing Stage}: the experiment generated data and the logs are uploaded to the Results Store. The experiment data is cleared from the local store and containers are removed. Finally, the executor sends a request to the orchestrator to kill the measurement server (if any). 

\projectname{}'s current deployment consists of $7$ Starlink user terminals located in the UK ($3\times$), Spain($2\times$), and the US ($2\times$). The terminals are locally connected via routers (comes with the Starlink kit) to Azure Stack Edge (ASE) nodes~\cite{ase}, Intel NUC devices~\cite{intel_nuc}, and desktop machines located in university and research labs.

%The current testbed deployment consists of 7 Starlink user terminals, located in US, UK, and Europe. The deployment consists of diverse set of user terminals -- 2 premium, 1 RV, and 4 residential. The terminals are connected to Azure Stack Edge (ASE) nodes \fix{\cite{?}}, Intel NUC device \fix{\cite{?}}, and desktop machines located in university labs. 

%\begin{figure}[tbh]
%        \begin{center} \includegraphics[width=\columnwidth]{figures_dump/experiment-pipeline.png}
%                % \vspace{-0.15in}
%                \caption{\projectname{} experiment pipeline
%                }
%                \label{fig:experiment-pipeline}
%        \end{center}
%        % \vspace{-0.2in}
%\end{figure}

%\parab{Experiment cycle} Fig. \ref{fig:experiment-pipeline} summarizes the experiment cycle. The testbed user prepares a docker image of the experiment and pushes it to a central repository. The user then modifies the configuration file (YAML) to define experiment parameters (such as the name of the container image to be used, and other user-defined experiment parameters). In the next step, the CLI is used to define the experiment schedule (ex, cron job, trigger), client/server nodes on which to schedule the experiment, and whether to mark the experiment as overhead/no-overhead. The orchestrator verifies the experiment configuration to check for schedule conflicts, verify the trigger string, and schedules the experiment. Each execution of the experiment is called a "run". The users can monitor execution of the experiment by listing the status of the experiment runs (Scheduled, executing, finished). Once the run has finished executing, the user can use the CLI to download the experiment data and use it for analysis. 



==> results.tex <==
\section{Experiments and insights}
\label{sec:results}

In this section, we present initial results that contextualize the importance of a global-scale testbed and demonstrate the capabilities of \projectname{}. The performance predictors and video streaming experiments demonstrate how \projectname{} could drive LEO innovation.
%\lc{would we talk about two dishes colocated experiments and insights here?}

\subsection{Latency and transport performance}
\label{subsec:latency_transport_results}

% First, we understand LEO's (currently SpaceX Starlink) latency offering by reaching out to popular public Internet services like DNS and CDN. \ns{Make this case: CDN and DNS are designed for low latency access. To obtain a lower bound on the latency offered by Starlink, we ask what latency we experience when accessing these services. Can we also say we do htis continuously to understand variability in latency?} We also compare how different popular congestion control schemes fare over these dynamic networks when compared against the terrestrial Internet. To reduce the footprint of our experiments\ns{seems lame to blame footprint of DNS lookup:) CDNs are also designed to take huge loads; we are unlikely to cripple these services. Just say we pick one client per country. no need ot give details}, we pick one of our measurement clients per country (Redmond or \textbf{RDM} in the US, Barcelona or \textbf{BCN} in Spain, and London or \textbf{LDN} in the UK) and run these experiments for a few hours still highlighting the key findings. \projectname{} is capable of running experiments $24${}$\times${}$7$ leveraging fully dedicated nodes and the scavenger mode on volunteer nodes.

% \begin{figure}[t]
%   \centering
%   \subfigure[]{\label{fig:dns_cloud_lat_cdf}
%     \includegraphics[width=0.4\textwidth]{figures/results/latency_data/google_dns_latency_cdf.png}}
%   \subfigure[]{\label{fig:redmond_cdn_cdf}
%     \includegraphics[width=0.25\textwidth]{figures/results/latency_data/redmond_cdn_cdf.png}}
%   \subfigure[]{\label{fig:akamai_cdf}
%     \includegraphics[width=0.25\textwidth]{figures/results/latency_data/akamai_cdf.png}}
%   \vspace{-0.2in}
%   \caption{Latency to (a) Google's $8$.$8$.$8$.$8$ from different locations, (b) Web domains fully hosted by popular CDNs from Redmond, and (c) Web domains hosted by Akamai from different locations.}
%   \vspace{-0.1in}
% \end{figure}

% \begin{figure*}[tbh]
%   \centering
%   \subfigure[]{\label{fig:latency_time_series}
%     \includegraphics[width=0.32\textwidth]{figures/results/latency_data/15mins_T2.png}}
%       \subfigure[]{\label{fig:leo_path}
%     \includegraphics[width=0.32\textwidth]{figures/design/LEO_path.png}}
%   \subfigure[]{\label{fig:latency_bar_plot}
%     \includegraphics[width=0.32\textwidth]{figures/results/latency_data/latency_bar_plot.png}}
%   \vspace{-0.2in}
%   \caption{(a) Latency varies over time with prominent spikes that persist for a while. (b) The individual color-coded segments of the path. S$2$ or the bent-pipe portion contributes the maximum latency. (c) The segment(S)-wise median latency for the end-to-end path to Google's DNS server.}
%   \vspace{-0.1in}
% \end{figure*}

% \parab{Latency to public DNS and CDNs} 
% We measure the \texttt{ping} and \texttt{hping} (TCP SYN-SYN/ACK handshake) latencies to popular DNS and CDN services from each of the $3$ locations RDM, BCN, and LDN for $6$ hours on the same day ($12^{th}$ Feb'$23$) and time. Fig.~\ref{fig:dns_cloud_lat_cdf} plots the CDFs of ping latencies to Google's anycast DNS servers ($8$.$8$.$8$.$8$)~\cite{google_dns}. The minimum and maximum median latencies to Google DNS are $34.8$~ms (RDM) and $35.3$~ms (LDN) respectively. Interestingly, at all of these locations, the latencies have long tails with the $99^{th}$ percentiles (worst latencies) being $>${}$2\times$ ($7$-$10\times$) the median. 
% %The median latencies to Google Cloud are \fix{$55.6$~ms for BCN and $41.8$~ms for LDN} with similar observations for the long tails. 
% We observe similar trends with \texttt{hping} and with Cloudflare's DNS ($1$.$1$.$1$.$1$)~\cite{cloudflare_dns}. In the latency time-series analysis below, we deep-dive into the long-tail latencies observed over Starlink's LEO network.

% We get the top Web domains from the Tranco list~\footnote{Available at https://tranco-list.eu/list/LY344 (generated on $04$ Dec, $2022$)}~\cite{tranco}, get the final redirected domains, filter domains (TLDs: com, net, edu, org, tv, io, site, gov), get corresponding IP addresses, and get the OrgName and NetName from \texttt{whois}~\cite{whois} registry to identify top $100$ sites fully served by (IP addresses belong to the CDN) $3$ popular CDN services -- Akamai, Cloudflare, and Fastly. \ns{why these specific CDNs. can you find some ref that these are the largest 3 or if we can say these are top 3 among the CDNs we find?} Fig.~\ref{fig:redmond_cdn_cdf} plots the CDFs to these $3$ CDNs from RDM. Fastly and Cloudflare has comparable performance with the median latency being the same for both -- $34.5$~ms. Latency to Akamai-hosted servers is $81\%$ higher at the median. Repeated tests show similar trends. Note that this inflated latency is specific only to RDM. As Fig.~\ref{fig:akamai_cdf} shows, the median latencies to Akamai domains are much lower at LDN ($34.2$~ms) and BCN ($36.6$~ms) and are comparable to Fastly and Cloudflare (plot omitted for brevity). %In \S\ref{subsec:app_experiments} we quantify the differences, if any, in Web browsing performance for these $3$ CDN services in RDM and the same set of Web pages (full-site delivery).

% %Fig.~\ref{fig:cdn_lat_cdf} plots the CDFs of ping latencies to these top domains. While the latencies to the CDN services are comparable at the median (with Fastly and Cloudflare offering slightly lower latencies than Akamai), Akamai latencies are \fix{$114\%$ (BCN) and $22.5\%$ (LDN) higher than Fastly at the $95^{th}$ percentiles.} In \S\ref{subsec:app_experiments} we quantify the differences, if any, in Web browsing performance for these $3$ CDN services and the same set of Web pages (full-site delivery).}

% %\parab{LEO vs. Internet latency} \fix{To be written.}
% From the BCN node (which also has direct access to the terrestrial Internet) we conducted the same CDN full-site delivery latency measurements. While for this location, median latencies over Starlink to the CDN-hosted domains are comparable ($34.2$ - $36.6$~ms) across Fastly, Cloudflare, and Akamai, over the terrestrial Internet Cloudflare offers lower median latency ($2.6$~ms) compared to Fastly ($14.5$~ms) or Akamai ($12.9$~ms). Fig.~\ref{fig:BCN_LEO_CDN} and \ref{fig:BCN_terrestrial_CDN} in the appendix show these latency plots.

% %\begin{figure}[]
% %        \begin{center} \includegraphics[width=\columnwidth]{figures/results/latency_data/15mins_T.png}
% %                \vspace{-0.15in}
% %                \caption{Latency varies over time with prominent spikes that persist for a while.
% %                }
% %                \label{fig:latency_time_series}
% %        \end{center}
% %        \vspace{-0.2in}
% %\end{figure}

% \parab{Latency time-series} Fig.~\ref{fig:latency_time_series} plots the ping latency to Google's $8$.$8$.$8$.$8$ from the BCN node for a period of $15$~min picked at random from the $6$ hour measurement window. While the observed median latency is $35.2$~ms for the larger window, we can see in this $15$~min granularity a few spikes with reported latencies larger than $70$~ms ($2\times$ the median) each persisting for roughly $15$ seconds or more. The first large spike starting at the $523^{rd}$ second of the window lasts for $30$ seconds. We speculate such high latencies occur due to sub-optimal hand-offs that last for multiples of $15$ seconds~\cite{15sec_1, 15sec_2} \ns{lets use Mohamed's script and show we would expect handoffs for this. Also, Mohamed: do we not talk about this in our IMC paper from last year? }. Interestingly, there are many smaller spikes with peak latencies around $50$~ms throughout, and the ping latencies change continually reflecting the LEO dynamics. Such highly dynamic behavior might translate to transport and application performance bottlenecks. Nevertheless, the high predictability of satellite trajectories also motivates us to build LEO latency predictors that we discuss in \S\ref{subsec:leo_prediction}. We also observe transient packet loss happening exactly when the spikes start/end. %Nevertheless, we do not find, in general, any correlation between latency and loss.

% \parab{Dissecting LEO bent-pipe latency} We run traceroutes from BCN, LDN, and RDM to Google's $8$.$8$.$8$.$8$ DNS server for $6$ off-peak hours of the day (midnight--6AM local time in each node) . Across $2588$ traces on average per location, we measure the individual segment(S)-wise one-way latency and plot the medians in Fig.~\ref{fig:latency_bar_plot}. Segment S$1$ is the user's private network behind the user terminal, S$2$ is the user terminal to satellite to terrestrial gateway bent-pipe, S$3$-S$5$ are Starlink internal network segments (verified by mapping IPs to ASNs), and S$6$ is the Internet part as demonstrated in Fig.~\ref{fig:leo_path}. As evident from Fig.~\ref{fig:latency_bar_plot}, the bent-pipe (S$2$) contributes the largest component to the end-to-end path latency -- $48\%$ for RDM and $54\%$ for both BCN and LDN at the median. Note that the bent-pipe latency should be highly predictable given the predictable LEO satellite trajectories. This is reflected when we predict the LEO path latency in \S\ref{subsec:leo_prediction} -- we achieve reasonably high accuracy even though the path includes terrestrial components. We leverage \texttt{trigger-based scheduling} to run traceroute probes from the LDN node to Google's DNS server when the path latencies are greater than the $95^{th}$ percentiles in the above measurement. We find S$2$ to contribute $\sim${}$77\%$ (at the median) of the higher end-to-end latencies. Given that bent-pipe latency is influenced by satellite positions relative to user terminals and terrestrial gateways, this observation motivates us to build an LEO latency predictor in \S\ref{subsec:leo_prediction}.

% %\fix{Also discuss trigger-based scheduling + traceroute.}

% %\begin{figure}[t]
% %  \centering
% %  \subfigure[]{\label{fig:}
% %    \includegraphics[width=0.8\columnwidth]{figures_dump/color_coded_median.jpg}}\\
% %    \vspace{-0.1in}
% %  \subfigure[]{\label{fig:}
% %    \includegraphics[width=0.8\columnwidth]{figures_dump/color_coded_95th.jpg}}
% %  \vspace{-0.2in}
% %  \caption{MK:I will still draw the path color coded as well}
% %  \vspace{-0.1in}
% %\end{figure}

% %\fix{Mention that we leveraged scavenger mode.}
% \begin{comment}
% \begin{figure}[t]
%   \centering
% \includegraphics[width=0.5\textwidth]{figures/results/congestion_control/throughput_cdf_google_numflows_1_window_combined.png}
%   \caption{Congestion control schemes suffer heavily due to LEO dynamics compared to their terrestrial counterparts.}
%   \label{fig:cc_comparison}
% \end{figure} 
% \end{comment}

% \begin{figure}[t]
%   \centering
%   \subfigure[]{\label{fig:cc_comparison}
%     \includegraphics[width=0.28\textwidth]{figures/results/congestion_control/throughput_cdf_google_numflows_1_window_combined.png}}
%   \subfigure[]{\label{fig:grpc_tput_comparison}
%     \includegraphics[width=0.34\textwidth]{figures/results/terminal_data/tput_comparison_ts.png}}
%   \subfigure[]{\label{fig:grpc_mae}
%     \includegraphics[width=0.34\textwidth]{figures/results/terminal_data/mae.png}}
%   \vspace{-0.2in}
%   \caption{(a) Congestion control schemes suffer heavily due to LEO dynamics compared to their terrestrial counterparts. Terminal-captured consumption data (b) temporally lag behind the experiment data and (c) need a time-shift correction of $1$ second (minimum mean absolute error across shifts).}
%   \vspace{-0.2in}
% \end{figure} 

% \parab{Congestion control showdown} At the BCN node, we ran \texttt{iperf}~\cite{iperf} upload tests to a Google cloud-hosted \texttt{e$2$-medium}~\cite{google_e2medium} server in Madrid (offering $2$~Gbps bandwidth) to compare the performance (goodput) of loss-based (Cubic~\cite{ha2008cubic}, NewReno~\cite{floyd2004newreno}) and delay-based (BBRv$1$~\cite{bbr}) transport over Starlink and the terrestrial Internet. Past simulations~\cite{kassing2020exploring} highlight the congestion-control (CC) performance bottlenecks in LEO arising due to continually changing latencies and hand-offs (latency spikes \& transient loss). To validate these findings, we ran each CC in $5$~min slots (interleaved) for a period of $30$~min over both LEO and the Internet. With a UDP burst test, we observed the maximum achievable upload speed over LEO to be $40$~Mbps and accordingly capped the terrestrial capacity (using \texttt{tc}~\cite{tc}) at this value.

% % percentages with respect to 40Mbps. 
% % median values: 
% % BBRv1-Terrestrial: 38/40 = 95 
% % BBRv1 19/40 = 48
% % NewReno 9/40 = 23
% % Cubic 11/40 = 28
% Fig.~\ref{fig:cc_comparison} shows that CC performance over LEO is significantly worse than over the terrestrial Internet. While terrestrially BBRv$1$ could achieve a median goodput of $95\%$ the capacity, over Starlink LEO, it could only achieve $48\%$. Loss-based schemes like Cubic and NewReno perform even worse, with median goodput reaching only $28\%$ and $23\%$ of the capacity respectively. Our observations are broadly in-line with \cite{kassem2022browser} where the tests were conducted over Starlink downlinks. Values in Fig.~\ref{fig:cc_comparison} larger than UDP burst goodput are reflections of the non-determinism of how \texttt{iperf} computes it.

% % \begin{figure}[t]
% %   \centering
% %   \subfigure[]{\label{fig:grpc_azimuth_elevation}
% %     \includegraphics[width=0.8\columnwidth]{figures/results/terminal_data/frequency_heatmap.png}}\\
% %     \vspace{-0.1in}
% %   \subfigure[]{\label{fig:grpc_orientation_latency}
% %     \includegraphics[width=0.8\columnwidth]{figures/results/terminal_data/95thptile_latency_heatmap.png}}
% %   \vspace{-0.2in}
% %   \caption{Heatmaps of (a) frequency of occurrence and (b) $95^{th}$ percentile latencies for combinations of antenna physical azimuth and elevation for the measurement client in Barcelona for $320+$ hours at a cadence of $1$ second.}
% %   \vspace{-0.1in}
% % \end{figure} 

\subsection{User terminal data analysis}
\label{subsec:terminaldata}

The user terminals (currently Starlink) at the measurement clients have an inbuilt telemetry system that continually monitors the physical orientation of the terminal (antenna), packet drop rate to PoP (point of presence on the other side of the bent-pipe last mile), ping latency to PoP, etc. While we have already discussed in \S\ref{sec:implementation} how \projectname{} consumes this data, here we touch upon the freshness of the terminal data and discuss some of the interesting correlations between terminal orientation and the network performance. %For the terminal data analyses, we pick one of our measurement clients deployed in Barcelona.

\begin{comment}
\begin{figure}[t]
        \begin{center} \includegraphics[width=0.75\columnwidth]{figures/results/terminal_data/tput_comparison_ts.png}
                \vspace{-0.15in}
                \caption{Terminal-captured consumption data temporally lag behind the experiment data.
                }
                \label{fig:grpc_tput_comparison}
        \end{center}
        \vspace{-0.3in}
\end{figure}
\begin{figure}[h!]
        \begin{center} \includegraphics[width=0.75\columnwidth]{figures/results/terminal_data/mae.png}
                \vspace{-0.15in}
                \caption{Terminal-captured consumption data need a time-shift correction of $1$ second (minimum mean absolute error across shifts).
                }
                \label{fig:grpc_mae1}
        \end{center}
\end{figure}
\end{comment}

\parab{Freshness of the terminal data}
We ran an \texttt{iperf} download test to the LDN node from a cloud server and collected both the iperf logs and the terminal-generated logs annotated with timestamps. We collected the data at a granularity of $100$~ms, and the plots in Fig.~\ref{fig:grpc_tput_comparison} compare the time-series consumption reports from both sources aggregated at the granularity of seconds. We see a phase shift between the plots with the terminal data lagging behind the iperf data in clock time. To quantify the time shift, we left-shift the terminal data in time and measure the mean absolute error between the $2$ time-series data. Fig.~\ref{fig:grpc_mae} shows that the error is minimum for a time correction of $1$ second. Note that this observation is stable across multiple client locations, and the location of the server does not matter in this context. The finding implies that terminal-provided consumption data is $1$ second stale. Hence, with scavenger mode, that leverages this zero-overhead terminal data, the user experience might see a transient dip for $1$ second as \projectname{} preempts/reschedules experiments. Note that while terminal-generated latency data shows a similar time shift, the physical orientation data (azimuth, elevation) is updated in real-time. The observations are stable across other locations.

Fig.~\ref{fig:grpc_mae} shows that the minimum mean-absolute error observed across different time shifts is $\sim${}$5.6$~Mbps. This is the header overhead that iperf does not account for~\cite{iperf_issues}. To minimize this gap, \projectname{}'s scavenger mode feature compares terminal-logged consumption data with the experiment container-level consumption data and reacts to temporal changes in the difference of the $2$ values rather than the absolute value of this difference.
%https://www.iwl.com/idocs/does-iperf-tell-white-lies

\begin{figure}[t]
  \centering
  \subfigure[]{\label{fig:grpc_azimuth_elevation}
    \includegraphics[width=0.4\textwidth]{figures/results/terminal_data/frequency_heatmap.png}}
  \subfigure[]{\label{fig:grpc_orientation_latency}
    \includegraphics[width=0.4\textwidth]{figures/results/terminal_data/95thptile_latency_heatmap.png}}
  \vspace{-0.2in}
  \caption{Heatmaps of (a) frequency of occurrence and (b) $95^{th}$ percentile latencies for combinations of antenna physical azimuth and elevation for the measurement client in Barcelona for $320+$ hours at a cadence of $1$ second.}
  \vspace{-0.3in}
\end{figure} 

% \parab{Temporal changes in terminal orientation} The measurements here have been collected for $320+$ hours from the BCN node in the last week of Dec'$22$ and the first week of Jan'$23$ \ns{Please update ot more recent measuerments} at a granularity of $\sim${}$1$ second. The physical orientation of the user terminal (antenna) seldom changes -- $90\%$ of the azimuth and elevation values lie within narrow bands of [$0.2$, $1.8$] (possibly to avoid GEO-arcs) and [$64.5$, $65.4$] degrees  respectively. %\lc{should we talking about the physical meaning of azimuth and elevation range? Azimuth [$0.2$, $1.8$]  means that starlink dish usually targets north which is claimed to be aviod interfernce from GEO satellite located on equatorial \cite{target_north}. Elevation [$64.5$, $65.4$] is design to maximize dish's visibility and cover area. } 
% Fig.~\ref{fig:grpc_azimuth_elevation} shows a few clusters of popular azimuth and elevation combinations with a long tail of other values. Note that the antenna changes its azimuth and elevation gradually, albeit at a slow median pace of $0.0001\degree$ per second for both axes. We do not have visibility into the phased-array beam~\cite{phased_array_unknown} orientation on top of the physical orientation of the antenna, but as we see next, the physical orientation could have important network performance implications.

% \parab{Some orientations could be worse!} 
% Fig.~\ref{fig:grpc_orientation_latency} plots the heatmap of $95^{th}$ percentile latencies for different combinations of terminal azimuth and elevation. The deepest hues (largest values of latency, still less than $100$~ms though) correspond to less popular orientations (see Fig.~\ref{fig:grpc_azimuth_elevation}). This has multiple important implications as we list below:
% \vspace{-0.05in}
% \begin{itemize}[leftmargin=*]
%     \item This observation motivates us to try and build an LEO latency estimator (also, a throughput estimator) with features that include terminal-generated data like azimuth, elevation, etc. in conjunction with other features like publicly available satellite trajectory data. We discuss in \S\ref{subsec:leo_prediction} this latency predictor that achieves an accuracy of $94.5\%$.
%     \item \projectname{}'s trigger-based scheduling functionality leverages such correlations if needed by experiments. The antenna orientation changes slowly ($0.0001\degree$ per second at the median) and hence provides the scheduler with leeway in triggering/rescheduling latency-dependent experiments as needed.
%     \item The community understands~\cite{bitag_latency} how the higher percentiles of latency impact application performance and user experience. Applications in the future could be able to predict LEO latencies for different end-points and react (application-level mitigations like right-sizing the jitter buffer for live video conferencing) accordingly.
% \end{itemize}
% \vspace{-0.05in}
% While we do not have access to the phased-array beam azimuth and elevation, the observation above pushes us to conjecture that some physical orientations only allow sub-optimal beam orientations. Such a phased array beam could be formed with a satellite far away from both the user terminal and the terrestrial gateway.

\parab{Outage and loss} For this entire period of $320+$ hours, we could see that the terminal was down (terminal state data) for $4$~min $52$~sec ($\sim${}$0.025\%$ of the time) in aggregate. We could not find any correlation between the physical orientation of the antenna and downtime. The same holds true for the ping drop rate to PoP.

\parab{Latency-versus-loss} In the terminal-generated data (BCN, $320+$ hours)\ns{this was done for BCN because we did not have time. do we now have data for all nodes?} above, we did not find any correlation (Pearson correlation score: $0.02$) between the observed loss rate and ping latencies to PoP. This observation is broadly in-line with our active measurements.

% \subsection{Toward predicting LEO performance}
% \label{subsec:leo_prediction}

% The observation in \S\ref{subsec:terminaldata} that some user terminal orientations could lead to higher $95^{th}$percentile latencies, the latency spikes that we see in Fig.~\ref{fig:latency_time_series}, and the observation in Fig.~\ref{fig:latency_bar_plot} that the bent-pipe adds the largest component to the end-to-end latency, entice us to believe LEO network performance could be predicted to a reasonable degree. Satellite trajectories are predictable over time -- publicly available satellite TLEs (two-line elements)~\cite{celestrak} define these trajectories for the next tens of hours and are updated regularly. Hence, the delay component driven by the satellite trajectories and gateway locations is predictable.

% %Hence, the delay that is influenced by these trajectories, frequent hand-offs between satellites, the orientation of the terminal, locations of gateways, etc. could be predicted, if not the component due to congestion.

% %\fix{Both are simple algorithms, so need to motivate why these specific algorithms. Also why these features are good/strong for prediction of latency/throughput.}
% We tried $2$ algorithms -- XGBoost~\cite{xgboost} (Extreme Gradient Boosting; Python's scikit-learn) and moving average forecasting (baseline). XGBoost is a gradient-boosted decision tree-based algorithm widely used for classification and regression. We use XGBoost for this regression problem as it can effectively handle non-linear relationships between the features (we describe below) and the target variable (latency). Moreover, it is an ensemble learning method that combines the predictions of multiple decision trees, leading to improved accuracy and stability. Moving average, on the other hand, is a simple time-series analysis technique that is particularly useful for handling noisy or unstable data, like the historic latency data in this case. We use the following features to train the predictor -- $1$. the terminal location coordinates (latitude, longitude, altitude), $2$. publicly available satellite trajectory information that gives the instantaneous locations (azimuth, elevation, and distance from the user terminal) of all satellites within the field of view of the user terminal, $3$. the user terminal orientation data (azimuth \& elevation),  $4$. the historic (last $5$ seconds) latency data recorded by the user terminal, and $5$. the time (timestamp in second). Across multiple locations (BCN in Spain, LDN in the UK, and San Diego, California or SD in the US), we train the models on $48$ hours of data at a granularity of $1$ second and test them with $\sim${}$5$ hours of data at the same granularity. We predict end-to-end latencies to servers hosted on geographically closest Azure locations.

% For locations that we tested, the model achieves a minimum mean accuracy of $94.5\%$ and performs consistently better than the baseline moving average forecasting at the median, $95^{th}$, and $99^{th}$ percentiles. The Relative Root Mean Square Percentage Error (RMSPE) and the Mean Absolute Percentage Error (MAPE) of the XGBoost model never exceed $10\%$ and $15\%$ respectively. We trained a similar model for predicting bandwidth albeit with a lower accuracy of $55\%$ due to larger variations.

% \begin{comment}
% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|cccc|cccc}
% \hline
% \textbf{ Testbed}               & \multicolumn{4}{c|}{XGBoost}    & \multicolumn{4}{c}{Harmonic Mean} \\  
% \textbf{ Location}               & MSE            & RMSE & $5\%$ & $10\%$  & MSE            & RMSE & $5\%$ & $10\%$\\  \hline
% \textbf{UK} & 0.03 & 0.05 &95.96 & 99.06 & 0.06 & 0.12 & 84.99\% & 92.92\% \\
% \textbf{SPAIN}  & 0.03 & 0.05 &96.84 & 99.3 & 0.06 & 0.13 & 83.69\% & 91.33\% \\
% \textbf{US} & 0.10 & 0.56 & 68.91 \% & 83.21\%  &  0.16 & 0.54 & 50.47 \% & 64.81\%   \\  \hline
% \end{tabular}}
% \caption{Main features for latency predictor}
% \label{table:predictor_factor}
% \end{table}
% \end{comment}

% In practice, these lightweight models need to be retrained regularly to accommodate long-term evolution like the deployment of more satellites. We plan to improve the accuracy of the models further by ingesting weather data and the client cell-local diurnal patterns in demands over longer periods of time. Such models could augment today's transport and application-level optimizations by making them LEO dynamics aware. We demonstrate one such use case in \S\ref{subsec:app_experiments} where we augment a well-known ABR (adaptive bit-rate) video streaming algorithm with the bandwidth predictor.

%\lc{To learn the latency-spiky observed in figures \ref{fig:Scaling}, \ref{fig:Scaling2}, we use the XGBoost \cite{}. XGBosst is ensemble decision tree-based and commonly repoted as one of the most accurate learning algorithm for linear regression. Table \ref{table:predictor_factor} lists out the prediction features and the number of collected data for building the latency predictor. For different areas(UK, Spain, US), we collect location-specific data and train the predictor.}

%\lc{\textbf{Metrics}. We evaluate the prediction performance by the Root Mean Square Error (RMSE) and the relative Root Mean Square Percentage Error (RMSPE), that are the standard metrics in regression. Besides, we report the ±5\% and ±10\% accuracy [13], that are the percentage of models with predicted latency within the corresponding error bound relative to the measured latency.}

%\lc{\textbf{Result}.  The prediction accuracy by different predictors. Compared with the baselines, our predictor can consistetly achieves accurate prediction on various loacation. Specifically, on average, our latency predictor achieves 80\% accuracy, better than heretical meaning (75\%) on the three location. }

\subsection{Application performance over LEO}
\label{subsec:app_experiments}

We now evaluate how Internet application performance over LEO networks (Starlink). The first experiment compares CDN full-site delivery performance at RDM (where Akamai-hosted Web server latencies are observed to be higher in \S\ref{subsec:latency_transport_results}). The second experiment demonstrates how our custom-built LEO performance predictors could potentially boost user experience for video streaming.

\begin{figure}[t]
        \begin{center} \includegraphics[width=0.4\columnwidth]{figures/results/Web_browsing/Redmond_pltbysize.png}
                \vspace{-0.15in}
                \caption{At Redmond, Web page load performance (page load time or PLT by page size) for Fastly is the best at the median. \db{Should we remove this Web browsing plot and the corr. write up? Is it adding anything useful?}}
                \label{fig:redmond_web}
        \end{center}
        %\vspace{-0.2in}
\end{figure}
% \parab{Web browsing} 
% To evaluate the impact of different latencies to the different CDN services at RDM (Redmond), we loaded the same domains ($100$ per CDN) as in \S\ref{subsec:latency_transport_results} with \texttt{Browsertime} from \texttt{sitespeed.io}~\cite{browsertime} and recorded the page load times (PLT) and page sizes. Fig.~\ref{fig:redmond_web} plots the CDFs of \texttt{PLT/size} for the $3$ CDNs. Interestingly, while Fastly (with the lowest latencies) offers the lowest PLT/size at the median, Cloudflare with similar latencies falls short ($3\times$ higher than Fastly). Another interesting observation is that, while Akamai lags behind Fastly at the median ($67\%$ higher PLT/size), it performs better at higher percentiles. This could be due to multiple reasons -- differences in server response time, congestion control, initial congestion windows, etc. Akamai, for example, is known~\cite{akamai_higher_icwnd} to use larger initial congestion windows. Irrespective of the findings, we would like to highlight the untapped performance opportunity for Akamai at RDM and similar locations -- path latencies have multiplicative impact~\cite{bozkurt2017internet} on higher layer protocols. \projectname{} offers a platform to test such performance opportunities and bottlenecks over LEO at scale.
% %https://www.cdnplanet.com/blog/initcwnd-settings-major-cdn-providers/
% %\parab{Video streaming in the wild} \fix{To be written}

\parab{LEO-aware ABR video streaming} In \S\ref{subsec:leo_prediction} we built lightweight client-local LEO latency and through predictors with reasonable accuracy. Could we use these predictors to improve the performance of applications running over LEO networks? Toward understanding this broad opportunity, we run a simple video streaming experiment in $2$ of our deployment sites -- BCN in Spain, and SD in the US. We generate network traces using \texttt{iperf} and the terminal-generated data for $10$ hours at a granularity of $1$ second and use a similar setup as in \cite{pensieve_qoe} to run our video streaming tests -- an emulated LEO network over Mahimahi \cite{netravali2015mahimahi}, and a custom encoded video from Pensieve of $3$~min duration with $6$ qualities. The encoded bitrate ratio is $\sim${}$1.5$ between adjacent qualities and tracks. We use RobustMPC~\cite{yin2015control} (control-theoretic) as the ABR (adaptive bitrate) algorithm and measure the standard video streaming QoE metric~\cite{pensieve_qoe} across $100$ runs of each algorithm as described below.

We use $3$ variants of the MPC algorithm -- $1$. Default MPC (MPC-D): the default implementation that uses its own custom throughput predictor, $2$. LEO-aware MPC (MPC-L): uses the LEO throughput predictor we trained with client-local data, and $3$. MPC with Oracle (MPC-O): knows the throughput trace in advance. Across all locations and multiple runs, we observe MPC-O (a hypothetical upper-bound) outperforms the other schemes (improves QoE by $30\%$ at the median over the baseline MPC-D) consistently, which is along the lines of expectation. Interestingly though, MPC-L, backed by our custom-built LEO predictor, also consistently outperforms MPC-D by $25\%$ at the median and $23\%$ at the $95^{th}$ percentile.\looseness=-1
%Note that MPC-O, which is a hypothetical upper bound, improves QoE by \fix{$30\%$} at the median over the baseline MPC-D in our experiments.}

%\lc{The MAE and RMSE for bandwidth prediction is (0.4 MAE and 0.64 RMSE), outperform moving average (0.45 MAE and 0.75 RMSE) by 10\%.}

These early results open up a broad LEO research opportunity -- making end-to-end protocols and applications aware of LEO networks. Lightweight network performance predictors deployed at user terminals should be able to serve multiple applications simultaneously.

%\lc{In this section, we evaluate the impact of our proposed bandwidth prediction algorithm on the Quality of Experience (QoE) of Multimedia Player Controller (MPC) algorithms. To this end, we compare the QoE of three MPC algorithms: mpc\_default, mpc\_prediction, and mpc\_oracle.}

%\lc{Our proposed algorithm is a bandwidth prediction mechanism for Starlink satellite communications, which can predict the bandwidth with over 80\% accuracy. By integrating this prediction mechanism into MPC, we aim to improve the QoE metric.}

%\lc{We present the results in the form of cumulative distribution functions (CDFs) of the QoE metrics. The CDFs for the three algorithms are shown in Figure \ref{fig:cdf_qoe}.}

%\lc{The results depicted in Figure 1 demonstrate that the mpc\_oracle algorithm outperforms the other two algorithms, achieving the highest QoE for the majority of users. Meanwhile, our proposed algorithm (mpc\_prediction) provides a slightly lower QoE than mpc\_oracle, with a value of 1.01 compared to 1.07. Despite this, it still outperforms the mpc\_default algorithm, which has a QoE value of 0.85.}

%\lc{These results suggest that our proposed bandwidth prediction algorithm is a valuable addition to the MPC framework. It provides a better QoE compared to the mpc\_default algorithm, while still achieving a slightly lower QoE compared to the mpc\_oracle. Our work thus contributes to the advancement of the MPC field by introducing a novel approach to improve QoE through the use of bandwidth prediction.}

%    \begin{figure}[h]
%        \centering
%        \includegraphics[width=1\linewidth]{figures_dump/cdf_qoe.png}
%        \caption{Video streaming of different abr algorithm}
%        \label{fig:cdf_qoe}
%    \end{figure}

==> results_bckp.tex <==
\subsection{Observed latencies}
[All locations; $20$ hours of data]
\begin{itemize}
    \item Ookla latency [single/multiple connections]
    \item Ping (ICMP, TCP, UDP) latency to
    \begin{enumerate}
        \item Anycast DNS services (like $8$.$8$.$8$.$8$, $1$.$1$.$1$.$1$)
        \item CDN servers (anycast?)
        \item cloud servers (Azure, Google, AWS)
    \end{enumerate}
\end{itemize}

\subsection{Latency time series}
We should also have traceroute (annotated with timestamp) data for the period. [All locations; Continuous $6$ hours]


Starlink is a satellite-based internet service provider that utilizes a network of low Earth orbit satellites to provide high-speed internet connectivity to users. One of the key features of the service is its ability to seamlessly handover connections from one satellite to another every 15 seconds, ensuring that users have a consistent and reliable connection. However, this process can sometimes result in latency spikes, where the time it takes for data to be transmitted between the user's device and the satellite is temporarily increased. These spikes can last for a few milliseconds to a few seconds and can be caused by various factors such as distance and weather conditions. Overall, the handover process is an important aspect of Starlink's service, as it allows for a stable and uninterrupted connection for its users, while also maintaining a high level of performance.

    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/6hours.png}
        \caption{Change point analysis}
        \label{fig:Scaling}
    \end{figure}

The figure shows the latency of a Starlink internet connection over 6 hours in the UK testbed. The line on the graph shows the overall trend of latency over time, with the dots indicating the specific data points. The red circles on the graph represent the handover points, which occur every 15 seconds as Starlink seamlessly switches between different satellites. The handover points are easily identifiable by the red circles on the graph, and they occur at various intervals throughout the data set. Overall, the graph illustrates the performance of the Starlink connection, including the trade-off between maintaining a stable connection through handovers and the occasional latency spikes that can occur as a result.

Change point analysis [hand-off detection]

    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/Time-serious.png}
        \caption{Change point analysis}
        \label{fig:Scaling}
    \end{figure}
    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/Time-serious2.png}
        \caption{Change point analysis}
        \label{fig:Scaling2}
    \end{figure}


    In our evaluation of the Starlink satellite-based internet service, we measured the latency experienced by users during handovers, starting from 2022-12-05 14:36:13. The measurements were taken at 15-second intervals, and the results are illustrated in Figure \ref{fig:Scaling}. The x-axis of the graph represents time in real-time format, and the y-axis represents latency in milliseconds.

    The solid line in the graph shows the measured latency, with brief spikes visible during handovers. The dotted lines indicate when handovers occurred, which can be seen as the brief increases in latency due to the signal switching from one satellite to another. The handovers were occurred on 2022-12-05 14:36:28 and 2022-12-05 14:36:43. Despite these brief spikes, the overall latency is stable and under 30ms which is considered as good performance. This is a remarkable achievement considering that the handovers occur seamlessly every 15 seconds and in remote or hard-to-reach areas.

    Figure \ref{fig:Scaling} illustrates an additional example of a handover that took 45 seconds starting at 2022-12-05 14:43:58 and ends at 2022-12-05 14:44:43. As seen in the graph, the latency spikes during the handover period, but it still falls within an acceptable range. The data shows that handovers usually take a multiple of 15 seconds, which is in line with the assumsion that starlink do the handover every 15 seconds. 

 Analyze end-to-end paths (using traceroute) at change points [Could be an example of trigger-based scheduling albeit zero addl. overhead] can't do that before triger-based handover happened
    \item Across locations, how frequent are these hand-offs? [color coded segments; where color = $95$th ptile latency]

    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/Handover-frequency.png}
        \caption{handover frequency}
        \label{fig:Scaling3}
    \end{figure}

    Figure \ref{fig:Scaling2} illustrates the handover frequency in the tested location of UK. As seen in the graph, most handovers occurred within 15 seconds, with some variations depending on the location. The data shows that handovers which took 15 seconds occurred 114 times per day, 30 seconds handovers happened 13 times per day, and so on. Furthermore, we observed that handovers and latency spikes over 50ms only happened 187 times per day, which represents a very small fraction of the total number of handovers, as can be seen in the graph. This demonstrates the robustness of the Starlink handover mechanism in maintaining stable latency and minimizing interruption even in varying conditions. 
    
 Map change points to simulations by comparing relative changes in latencies to reverse engineer hand-offs?
    
\subsection{Latency Prediction}


\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c}
\hline
\textbf{Variable}               & \textbf{Features}            & \begin{tabular}[c]{@{}c@{}} \# Collected Data, \\  UK Spain US\end{tabular}                                                                      \\ \hline

Experimental data     &   $Latency_{t-1,t-2,t-3,t-4,t-5}$     & 2 days, 3 days, 3 days                                                                           \\ \cline{1-2}

Dish-specific data    &    \begin{tabular}[c]{@{}c@{}} $Latitude, longitude$, \\  $azimuth(dish)_t, elevation(dish)_t$\end{tabular}
     &               \\ \cline{1-2}

Simulation data    &   \begin{tabular}[c]{@{}c@{}} $azimuth(sat)_t, elevation(sat)_t$, \\  $distance(sat)_t$\end{tabular}
     &                \\ \hline
     
\end{tabular}}
\caption{Main features for latency predictor}
\label{table:predictor_factor}
\end{table}

\lc{
To learn the latency-spiky observed in figures \ref{fig:Scaling}, \ref{fig:Scaling2}, we use the XGBoost \cite{}. XGBosst is ensemble decision tree-based and commonly repoted as one of the most accurate learning algorithm for linear regression. Table \ref{table:predictor_factor} lists out the prediction features and the number of collected data for building the latency predictor. For different areas(UK, Spain, US), we collect location-specific data and train the predictor.}

\lc{
\textbf{Metrics}. We evaluate the prediction performance by the Root Mean
Square Error (RMSE) and the relative Root Mean Square Percentage
Error (RMSPE), that are the standard metrics in regression. Besides,
we report the ±5\% and ±10\% accuracy [13], that are the percentage
of models with predicted latency within the corresponding error bound relative to the measured latency.}

\lc{
\textbf{Result}.  The prediction accuracy by different predictors. Compared with the baselines, our predictor can consistetly achieves accurate prediction on various loacation. Specifically, on average, our latency predictor achieves 80\% accuracy, better than heretical meaning (75\%) on the three location. }



\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc|cccc}
\hline
\textbf{ Testbed}               & \multicolumn{4}{c|}{XGBoost}    & \multicolumn{4}{c}{Mean} \\  
\textbf{ Location}               & RMSE            & RMSPE & $5\%$ & $10\%$  & RMSE            & RMSPE & $5\%$ & $10\%$\\  \hline
\textbf{UK}               & \\
\textbf{SPAIN}               & \\
\textbf{US}               & \\  \hline
\end{tabular}}
\caption{Main features for latency predictor}
\label{table:predictor_factor}
\end{table}


\subsection{Latency under load}
[All locations; $5$ hours of data?; $15$-$25$ TCP connections in parallel]
\begin{enumerate}
    \item Anycast DNS services (like $8$.$8$.$8$.$8$, $1$.$1$.$1$.$1$)
    \item CDN servers (anycast?)
    \item cloud servers (Azure, Google, AWS)
\end{enumerate}

\subsection{Traceroute results}
[All locations; $20$ hours of data annotated with timestamps]
\begin{itemize}
    \item Find latency for each segment
    \item Compare segment-wise latencies across locations
\end{itemize}

\subsection{Throughput measurements}
Using Cong's pipeline/iperf/individual cc implementations.
[All locations; $5$min x $10$ slots per transport and config]
\begin{itemize}
    \item Transport: Cubic, NewReno, BBRv$1$, BBRv$2$, PCC, Copa, UDP, ...
    \item Config: $1$ flow, $15$ flows, $25$ flows
    \item To Azure cloud servers.
\end{itemize}

\subsection{Starlink gRPC bytes sent validation for Scavenger mode}
Cubic/NewReno $1$ flow vs. Starlink gRPC bytes sent.
[$3$ locations; $5$ min; could leverage the experiment above]

\subsection{Starlink gRPC ping-drops versus our latency/loss measurements}
[Could leverage latency and throughput experiments above]
\begin{itemize}
    \item Do ping drops correlate with latency/loss spikes?
\end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures_dump/Correlation between latency spikes and ping drop.png}
    \caption{Correlation between latency spikes and ping drop}
    \label{fig:Scaling}
\end{figure}
Correlation between latency spikes and ping drop is near zero.

\subsection{Starlink gRPC - time series data}
[All nodes, all the time; free data]

\begin{itemize}
    \item  azimuth and elevation states. Starlink dish is forced to target north (azimuth \approx 0, elevation \approx 70) 

Figure Azimuth histogram with loss: This histogram shows the distribution of azimuth angles and the corresponding loss rate (ping drop rate) for a satellite environment. The x-axis represents the range of azimuth angles, while the y-axis represents the frequency of the azimuth angles in the data set. The color of the histogram represents the ping loss rate, with red indicating high loss and green indicating low loss. This plot helps to visualize the relationship between azimuth angle and loss rate and identify any patterns or trends in the data.

Elevation histogram with loss: This histogram shows the distribution of elevation angles and the corresponding loss rate (ping drop rate) for a satellite link. The x-axis represents the range of elevation angles, while the y-axis represents the frequency of the elevation angles in the data set. The color of the histogram represents the loss rate, with red indicating high loss and green indicating low loss. This plot helps to visualize the relationship between elevation angle and loss rate and identify any patterns or trends in the data.

2D histogram with loss: This 2D histogram shows the relationship between azimuth and elevation angles, and the corresponding loss rate (ping drop rate) for a satellite link. The x-axis represents the range of azimuth angles, the y-axis represents the range of elevation angles, and the color represents the loss rate, with red indicating high loss and green indicating low loss. This plot helps to visualize the relationship between azimuth, elevation angles and loss rate and identify any patterns or trends in the data. It can also help to identify any specific azimuth and elevation angle ranges that have higher loss rates.
    
    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/direction_histgram.png}
        \caption{azimuth and elevation states}
        \label{fig:Scaling}
    \end{figure}

    \item Temporal changes in azimuth and elevation lead to lost connection (100\% ping drop and 0 ms latency)
    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/forced_movement.png}
        \caption{Temporal changes in azimuth and elevation}
        \label{fig:Scaling}
    \end{figure}


    \item Plot the above alongside ping-drop time series to identify repeating patterns [which could be physical obstructions]
    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/histgram.png}
        \caption{alongside ping-drop time series to identify repeating patterns}
        \label{fig:Scaling}
    \end{figure}
    \item Trigger-based scheduling example: When $azimuth = X + \epsilon$, $elevation = Y + \epsilon$, and the ping-drop rate increases, suspend execution and resume when the conditions improve.
\end{itemize}

\subsection{Profiling the Energy Consumption of Starlink dish}

Starlink RV provide IN-MOTION USE. Therefore it requires  an on-board power supply for usage.

%\begin{itemize}
% \item Energy Consumption for providing serverse. 
% \item Energy Consumption when it is downloading at full speed.
% \item Energy Consumption when it serves multiple users.
% \item Energy Consumption for residential and RV.
%\end{itemize}

\subsection{Web browsing}
top X pages from Tranco list
[All nodes, n iterations]
\begin{itemize}
    \item Metrics: viz$85$, SpeedIndex, page load time
    \item compare against terrestrial Internet
    \item Partition by no. of requests, page size, etc.
    \item filter for pages with CDN full-site delivery
    \item host the same on Azure, Google cloud, AWS and measure performance.
\end{itemize}

\subsection{Video streaming}
Popular streaming services, popular/recent ABR algorithms.

In this section, we evaluate the impact of our proposed bandwidth prediction algorithm on the Quality of Experience (QoE) of Multimedia Player Controller (MPC) algorithms. To this end, we compare the QoE of three MPC algorithms: mpc\_default, mpc\_prediction, and mpc\_oracle.

Our proposed algorithm is a bandwidth prediction mechanism for Starlink satellite communications, which can predict the bandwidth with over 80\% accuracy. By integrating this prediction mechanism into MPC, we aim to improve the QoE metric.

We present the results in the form of cumulative distribution functions (CDFs) of the QoE metrics. The CDFs for the three algorithms are shown in Figure \ref{fig:cdf_qoe}.

The results depicted in Figure 1 demonstrate that the mpc\_oracle algorithm outperforms the other two algorithms, achieving the highest QoE for the majority of users. Meanwhile, our proposed algorithm (mpc\_prediction) provides a slightly lower QoE than mpc\_oracle, with a value of 1.01 compared to 1.07. Despite this, it still outperforms the mpc\_default algorithm, which has a QoE value of 0.85.

These results suggest that our proposed bandwidth prediction algorithm is a valuable addition to the MPC framework. It provides a better QoE compared to the mpc\_default algorithm, while still achieving a slightly lower QoE compared to the mpc\_oracle. Our work thus contributes to the advancement of the MPC field by introducing a novel approach to improve QoE through the use of bandwidth prediction.

    \begin{figure}[h]
        \centering
        \includegraphics[width=1\linewidth]{figures_dump/cdf_qoe.png}
        \caption{Video streaming of different abr algorithm}
        \label{fig:cdf_qoe}
    \end{figure}


    

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc|cccc}
\hline
\textbf{ Testbed}               & \multicolumn{4}{c|}{XGBoost}    & \multicolumn{4}{c}{Harmonic Mean} \\  
\textbf{ Location}               & MSE            & RMSE & $5\%$ & $10\%$  & MSE            & RMSE & $5\%$ & $10\%$\\  \hline
\textbf{UK} & 0.03 & 0.05 &95.96 & 99.06 & 0.06 & 0.12 & 84.99\% & 92.92\% \\
\textbf{SPAIN}  & 0.03 & 0.05 &96.84 & 99.3 & 0.06 & 0.13 & 83.69\% & 91.33\% \\
\textbf{US} & 0.13 & 5.43 & 59.3 \% & 75.88\%  &  0.72 & 8.13 & 48.25 \% & 60.32\%   \\  \hline
\end{tabular}}
\caption{Main features for latency predictor}
\label{table:predictor_factor}
\end{table}


==> testbeds.tex <==
\section{Yet another testbed?}
\label{sec:testbeds}

%\projectname{} adds to the growing list of network measurement testbeds. So, why cannot we simply augment an existing globally deployed testbed instead of re-inventing the wheel or at least a large part of it? 
In this section, we touch upon some of the well-known measurement testbeds and discuss why it is still necessary to deploy \projectname{}.

\subsection{Existing testbeds \& their limitations}
Most of the existing testbeds are focused on terrestrial networks~\cite{bajpai2015survey} and do not have the necessary mechanisms to detect and react to the highly dynamic changes that occur in LEO satellite networks. While LEO broadband is still in its infancy, it is critical to quantify and understand its nuances well so that novel solutions across the network stack could unleash its full potential. Below, we review some widely used testbeds  and motivate the need for \projectname{}.

\parab{Fixed-network deployments} 
PlanetLab~\cite{planetlab2023web, chun2003overlay, peterson2003blueprint} served as a platform for developing and testing new network protocols and services on a global scale for the past couple of decades. Our objective is similar in spirit: to establish a ``PlanetLab for LEO broadband'' with a widespread presence across multiple regions. However, in our envisioned LEO testbed, the majority of measurement clients will be located in residential areas where LEO broadband serves as the primary source of connectivity. RIPE Atlas~\cite{atlas2023web} project aims at measuring global internet connectivity and reachability through clients (probes) and measurement servers (anchors). The probes, deployed by volunteers, can run standard network experiments like traceroute, ping, DNS, NTP, etc. Similar to the RIPE Atlas model, we could ship Raspberry Pi-based~\cite{rasp_pi} devices, if needed, to volunteers who then become measurement client nodes in our testbed. Nevertheless, measurement clients in \projectname{} are currently more powerful edge devices like Azure Stack Edge~\cite{ase}, Intel NUC~\cite{intel_nuc}, and standard workstations. The M-Lab~\cite{dovrolis2010mlab} runs a fixed set of carefully vetted experiments, mostly implemented on the server side (e.g., the network diagnostic tool or NDT~\cite{ndt}). The experiments are only  conducted when a user accesses the tool and opts to initiate a test. M-Lab servers are mostly deployed in data centers where last-mile ISPs interconnect and clients use browser plugins or specialized hardware. Other testbeds such as BISmark~\cite{sundaresan2014bismark} and SamKnows~\cite{samknows2023web} conduct broadband measurements  by sending specially instrumented WiFi routers to homes and volunteers. 

\parab{Wireless \& cellular deployments} The ORBIT~\cite{Orbit} project started in 2003 to create an open-access wireless testbed for the research community. The testbed has made a significant impact and has been widely used in research on MANET, mesh networks, DTN, media streaming over wireless networks, mobile content delivery, and wireless security. PhoneLab~\cite{PhoneLab}\cut{developed by a research team at the University of Buffalo,} consists of hundreds of smartphones, to create a unique environment for developing and testing  mobile technology on smartphones at scale. Monroe~\cite{alay2017monroe} testbed is a measurement testbed that is focused on cellular networks. Monroe's implementation bears a superficial similarity to our approach, as it is based on docker containers. However, Monroe does not include any of the unique features of \projectname{} we discuss next.


Given LEO's high dynamicity and upcoming advancements, such as inter-satellite laser links, there is a need for a testbed like \projectname{} whose design is specifically tailored to measure the performance of such networks. \projectname{} enables dynamic network experiments, utilizes data generated by user terminals, reacts to anomalous/dynamic changes in connectivity characteristics, and has the ability to operate in scavenger mode to prioritize user traffic as required. A logically centralized cloud orchestrator manages the scheduling problem at scale. 

\cut{
\parab{PlanetLab}~\cite{planetlab2023web, chun2003overlay, peterson2003blueprint}
\ns{was a widely used testbed for developing new network protocols and services and testing them on a planetary scale. \cut{PlanetLab was motivated by the idea that wide-area networking services being proposed by researchers had to be tested on a planetary scale.} We share a similar need for a wide presence across multiple geographic regions. Our goal is similar in spirit: to set up a ``PlanetLab for \cut{Starlink} \debopam{LEO broadband}'' which allows researchers to measure \cut{Starlink} \debopam{LEO} connectivity from a variety of vantage points across the globe. \debopam{However, unlike in PlanetLab, we envision an LEO testbed to have measurement clients that} are based in residential locations where they are often the primary source of connectivity. \debopam{Also, PlanetLab experiments could not} react to anomalous or dynamic changes in connectivity characteristics.}

\cut{However, we \cut{have} \debopam{need} a number of unique adaptations, such as the Trigger mode to react to anomalous or dynamic changes in connectivity characteristics. Unlike PlanetLab; many \projectname{} nodes are based in residential locations where they are often the primary source of connectivity, requiring the need for scavenger mode measurements. Eventually, we expect to move to a similar setup as PlanetLab whereby universities can contribute resources (a Starlink Terminal) and join \projectname{}.} 

\parab{RIPE Atlas}~\cite{atlas2023web} is operated by the RIPE Network Coordination Centre that is aimed at measuring internet connectivity and reachability globally. RIPE Atlas probes, deployed by volunteers, could run standard network experiments like traceroute, ping, DNS, NTP, etc. 


While \projectname{} also encompasses both measurement clients (similar to probes) and servers (similar to anchors), the platform is envisioned to allow dynamic network experiments, consume user terminal-generated data, and operate in scavenger mode (see \S\ref{subsec:unique}) to prioritize user traffic, as needed. A logically centralized cloud orchestrator manages schedules and conflicts online. Similar to the RIPE Atlas model, we ship Raspberry Pi-based devices~\cite{rasp_pi}, if needed, to volunteers who then become measurement client nodes in our testbed. \debopam{Nevertheless, measurement clients in \projectname{} could also be more powerful edge devices~\cite{ase} depending on the site of deployment.}

\parab{SamKnows}~\cite{samknows2023web} \ns{conducts broadband measurements (typically in conjunction with a regulator, such as FCC in the US or OfCom in the UK) by sending specially instrumented WiFi routers to homes. \cut{Many RIPE Atlas probes and all} All SamKnows probes (and many RIPE Atlas probes) are hosted in residential locations, which means having to deal with the possibility of disrupting connections if measurement tests are bandwidth-intensive. Both RIPE and SamKnows take the conservative approach of carefully screening tests and ensuring resource consumption is minimized. We take a different design approach that also allows for bandwidth-hungry experiments (e.g., \texttt{iperf})\cut{as well. This allows for a wider range of experiments} which are important to understand \cut{Starlink} \debopam{LEO network performance nuances}, but we need to do that in a controlled manner (through the scavenger mode discussed in \S\ref{subsec:unique}), so that the volunteer's connectivity needs are not degraded as a result.}

\parab{M-Lab}~\cite{dovrolis2010mlab} \ns{Similar to RIPE, M-Lab runs a fixed set of carefully vetted experiments, mostly implemented on the server-side (e.g., the network diagnostic tool \debopam{or NDT}, which is a version of a `speedtest'). This means the experiments are only run when a user accesses a tool and chooses to run a test. \debopam{M-Lab servers are mostly deployed in data centers where last-mile ISPs interconnect and clients use browser plugins or are specialized hardware.} Although M-Lab  benefits from tight integration\fix{~\cite{mlab_google}} with Google, which results in vast numbers of tests, it does not allow for timed tests \cut{such as} needed for measuring \cut{Starlink} \debopam{LEO network} dynamics.}

\parab{Monroe}~\cite{alay2017monroe} \ns{testbed is a measurement testbed that is focused on cellular networks. The implementation bears a superficial similarity to our approach, as it is based on docker containers. \debopam{Monroe does not include any of the unique features of \projectname{} we discuss next.}}

\parab{Orbit}~\cite{Orbit} The ORBIT project started in 2003 to create an open-access wireless testbed for the research community. The testbed has made significant impact and been widely used in research on MANET, mesh networks, DTN, media streaming over wireless networks, mobile content delivery, and wireless security. 

\parab{PhoneLab}~\cite{PhoneLab} A research team at University of Buffalo developed PhoneLab, which consists of hundreds of smartphones, to create a unique environment for developing and testing  mobile technology on smartphones at scale. It opened for public experiments in 2013 and has got great responses since then. Neither Orbit nor PhoneLab targets LEO scenarios, where satellites constantly moving and the signal propagates between the earth and space. 
}

%\projectname{} stands on the shoulders of giants -- learns from their design choices and builds unique LEO-specific features to make the most out of the proposed testbed. We welcome community feedback on how already existing testbeds could embrace these features and absorb \projectname{}.

\subsection{\projectname{}'s unique features}
\label{subsec:unique}

While we delve into the detailed design and implementation of \projectname{} in \S\ref{sec:design}, here we touch upon the unique \projectname{} features that help us dissect LEO network subtleties and make the testbed deployable at scale.

\parab{Ingesting user terminal data} The Starlink user terminals run continuous measurements in the background and collect bent-pipe latency, traffic volume, packet loss, antenna directional data, etc. These statistics are made available to the private network behind the user terminal via gRPC APIs~\cite{starlink_grpc}. \projectname{} has the capability to continually gather this data, near real-time, and generate insights locally at the measurement client, such that the client could autonomously make decisions that enable the following two unique capabilities of the testbed. \cut{Note that we did not observe any PII in this terminal-generated data at the time of writing this paper}. In \S\ref{subsec:terminaldata} we conduct an analysis of the freshness and accuracy of this Starlink gRPC data.

\parab{Scavenger mode} This unique feature allows \projectname{} to locally (at the measurement client) preempt and reschedule experiments that result in upload/download traffic overhead when user traffic is sensed. This makes \projectname{} truly scalable -- volunteers across the globe with access to user terminals could join the testbed and contribute compute/connectivity free-cycles to the testbed. By leveraging the terminal-provided data that comes with no additional overhead, \projectname{} could locally sense (higher-priority) user traffic and preempt/reschedule experiments as needed. In \S\ref{sec:discussions}, we discuss how we plan to engage volunteers in this global measurement effort and make sure that the data consumption overhead due to \projectname{} experiments stays within data-capping bounds. One of \projectname{}'s current measurement clients in the UK is run as a volunteer node on which we successfully tested scavenger mode.

\parab{Trigger-based scheduling} Individual experiments on \projectname{} could specify triggers. For example, an experiment might say, ``\textit{if current network latency $>$ $10\times$ the moving average (of network latency) of last ten windows, trigger traceroute probes to Google's $8$.$8$.$8$.$8$ service}''. The experiment could run locally, at the client, and register its trigger with an autonomously running module at the measurement client that continually consumes the terminal data and checks if the condition is met. The experiment is notified of the current status of the condition in real time. We demonstrate this feature while discussing LEO bent-pipe latency under \S\ref{subsec:latency_transport_results}. In the future, we plan to make these triggers more diverse -- experiments can be enabled to specify conditions that take into account publicly available satellite trajectory information, local weather data, etc.

%\parab{} It is non-trivial to design a global-scale LEO testbed that could offer useful features like the scavenger mode and trigger-based scheduling. Also, this paper hides the complex logistics related to the procurement, shipment, and deployment of the terminals. We discuss the scalability and cost implications under \S\ref{sec:discussions}.


